PAGURUS: Low-Overhead Dynamic Information Flow Tracking on Loosely Coupled Accelerators

Software-based attacks exploit bugs or vulnerabilities to get unauthorized access or leak confidential information. Dynamic information flow tracking (DIFT) is a security technique to track spurious information flows and provide strong security guarantees against such attacks. To secure heterogeneous systems, the spurious information flows must be tracked through all their components, including processors, accelerators (i.e., application-specific hardware components) and memories. We present PAGURUS, a flexible methodology to design a low-overhead shell circuit that adds DIFT support to accelerators. The shell uses a coarse-grain DIFT approach, thus not requiring to make modifications to the accelerator's implementation. We analyze the performance and area overhead of the DIFT shell on FPGAs and we propose a metric, called information leakage, to measure its security guarantees. We perform a design-space exploration to show that we can synthesize accelerators with different characteristics in terms of performance, cost and security guarantees. We also present a case study where we use the DIFT shell to secure an accelerator running on a embedded platform with a DIFT-enhanced RISC-V core.

==> Makefile <==
# Makefile

# .tex file
PAPER = paper

# .bib file
REFS = refs.bib

# tex compiler
LATEXCC = pdflatex

# epstopdf script
export EPSTOPDF=epstopdf

# Dependencies

# .tex files
TEX_DEPS = $(wildcard $(PAPER).tex)   \
           $(wildcard sections/*.tex) \
           $(wildcard results/*.tex)

# .pdf files
FIG_DEPS = $(wildcard figures/pdfs/*.pdf)

# .gp files
GNU_DEPS = $(wildcard plots/info_leakage/gray/*.gp)  \
           $(wildcard plots/info_leakage/mean/*.gp)  \
           $(wildcard plots/info_leakage/mults/*.gp) \
           $(wildcard plots/fpga_execution/gray/*.gp)  \
           $(wildcard plots/fpga_execution/mean/*.gp)  \
           $(wildcard plots/fpga_execution/mults/*.gp) \
           $(wildcard plots/mem_overhead/gray/*.gp)  \
           $(wildcard plots/mem_overhead/mean/*.gp)  \
           $(wildcard plots/mem_overhead/mults/*.gp)

# Makefile rules

# main target
all: $(PAPER).pdf

# paper pdf generation
$(PAPER).pdf: gnu $(TEX_DEPS) $(FIG_DEPS) $(REFS)
	$(LATEXCC) $(PAPER)
	bibtex $(PAPER)	
	$(LATEXCC) $(PAPER)
	$(LATEXCC) $(PAPER)

# gnuplot graph generation
gnu: $(GNU_DEPS)
	echo "generating gnuplot"
	make -C plots/info_leakage/gray/ 
	make -C plots/info_leakage/mean/ 
	make -C plots/info_leakage/mults/ 
	make -C plots/fpga_execution/gray/ 
	make -C plots/fpga_execution/mean/ 
	make -C plots/fpga_execution/mults/ 
	make -C plots/mem_overhead/gray/ 
	make -C plots/mem_overhead/mean/ 
	make -C plots/mem_overhead/mults/ 

# cls generation for ACM
%.cls:   %.ins %.dtx
	pdflatex $<

# clean the generated file
clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf
	make clean -C plots/info_leakage/gray/ 
	make clean -C plots/info_leakage/mean/ 
	make clean -C plots/info_leakage/mults/ 
	make clean -C plots/fpga_execution/gray/ 
	make clean -C plots/fpga_execution/mean/ 
	make clean -C plots/fpga_execution/mults/ 
	make clean -C plots/mem_overhead/gray/ 
	make clean -C plots/mem_overhead/mean/ 
	make clean -C plots/mem_overhead/mults/ 
       
.PHONY: all clean gnu



==> sections/biblio.tex <==
%
% Bibliography
%

\bibliographystyle{ACM-Reference-Format}
\bibliography{refs}


